Quasi-Regression Monte-Carlo scheme for semi-linear PDEs and BSDEs with large scale parallelization on GPUs

In this article we design a novel quasi-regression Monte Carlo algorithm in order to approximate the solution of discrete time backward stochastic differential equations (BSDEs), and we analyze the convergence of the proposed method. The algorithm also approximates the solution to the related semi-linear parabolic partial differential equation (PDE) obtained through the well-known Feynman-Kac representation. For the sake of enriching the algorithm with high-order convergence a weighted approximation of the solution is computed and appropriate conditions on the parameters of the method are inferred. With the challenge of tackling problems in high dimensions we propose suitable projections of the solution and efficient parallelizations of the algorithm taking advantage of powerful many-core processors such as graphics processing units (GPUs).

==> Introduction21fev.tex <==
% !TEX root = ./template.tex


\section{Introduction}

\red{
Since the 1940s, Feynman-€"Kac formula has provided a probabilistic interpretation of the solutions of linear partial differential equations (PDEs). Thence, Monte Carlo method has become an alternative to deterministic numerical algorithms for solving linear PDEs. While traditional deterministic methods like finite differences, finite elements or finite volumes suffer from the so-called \textit{curse of dimensionality} \cite{bellmann} (i.e. as the dimension grows, the complexity of the algorithms grows exponentially), the rate of convergence of Monte Carlo methods does not depend on the dimension of the state space. As a consequence, in order to solve equations of dimension greater than $4$ or $5$, the probabilistic approach often remains the only numerical method available.

In the 1990s, the theory of backward stochastic differential equations (BSDEs) provided a probabilistic interpretation for non-linear problems. BSDEs are stochastic differential equations (SDEs) for which a terminal condition is specified and their solutions are pairs of processes. Linear BSDEs were introduced by Bismut \cite{bis:73} in 1973 in order to study stochastic control problems and their connections with the Pontryagin maximum principle of optimality. A rigorous study of BSDEs was started by Pardoux and Peng in 1990, who proved in  their seminal article \cite{pard:peng:90} the first well-posedness result for non-linear BSDEs, see also \cite{pard:peng:92}. These equations have the general form of
 \begin{align}
 -dY_t &= f(t,Y_t,Z_t) dt - Z_t dW_t, \nonumber \\
 Y_T &= \xi, \nonumber
\end{align}
where $0\leq t \leq T $, $(W_t)_{t\geq 0}$ is a Brownian motion, the terminal condition $\xi$ is a random variable, and the solution is a pair of adapted processes $(Y,Z)$.
The first applications of BSDEs in finance were conducted by El Karoui, Peng and Quenez \cite{elka:peng:quen:97} in 1997. They applied BSDEs in a European option pricing problem, where the randomness of $(Y,Z)$ comes from a forward SDE in $X$ as follows,
   \begin{align*}
     dX_t &= b(t,X_t) dt + \sigma(t,X_t) dW_t, \quad   X_0 = x_0,  \\
     -dY_t &= f(t,X_t,Y_t,Z_t) dt - Z_t dW_t, \quad  Y_T = g(X_T).
    \end{align*}
Now the terminal condition of the BSDE is determined by the stochastic terminal value of the FSDE through some deterministic function $g$. This system of SDEs, to which we will devote this article, is known as decoupled\footnote{Fully coupled FBSDEs have the general form   \begin{align*}
     dX_t &= b(t,X_t,Y_t,Z_t) dt + \sigma(t,X_t,Y_t,Z_t) dW_t, \quad   X_0 = x_0,  \\
     -dY_t &= f(t,X_t,Y_t,Z_t) dt - Z_t dW_t, \quad  Y_T = g(X_T).
    \end{align*}} forward-backward stochastic differential equation (FBSDE in short). It is also referred as Markovian BSDE, since the terminal condition of the BSDE and $f$ are random only through a Markov process. 
    
After the already mentioned celebrated work of El Karoui, Peng and Quenez, the interest in BSDEs has increased, mainly due to the connection of these tools with stochastic control and PDEs, connection that will be stated clearly soon. Let us start with a rigorous definition of the problem at hand.


}

\paragraph{The problem.}
In this work we are interested in numerically approximating the solution $(X,Y,Z)$ of a decoupled forward-backward stochastic differential equation
\begin{align}
%\begin{split}
\label{eq:fbsde}
Y_t& =  g(X_T) + \int_t^T f(s,X_s,Y_s,Z_s) \ds - \int_t^T Z_s \dW_s, \\
\label{eq:eds}
X_t & =  x + \int_{ 0} ^t b(s,X_s) \ds + \int_{0} ^t \sigma(s,X_s) \dW_s.
%\end{split}
\end{align}
The terminal $T>0$ is fixed. These equations are considered in a filtered probability space $(\Omega,\cF,\P,(\cF_t)_{ 0 \leq t \leq T})$ supporting a $q\geq 1$  dimensional Brownian motion $W$. The filtration is assumed to be the natural filtration of $W$ augmented with the $\P$-null  sets. In this representation, $X$ is a $d$-dimensional adapted continuous process (called the forward component), $Y$ is a scalar adapted continuous process and $Z$ is a $q$-dimensional progressively measurable process. Consideration of multi-dimensional $Y$ is quite straightforward and is discarded for the sake of simplicity. Regarding terminology, $g(X_T)$ is called \emph{terminal condition} and $f$ the \emph{driver}. Under standard assumptions (like $L^2$-integrability and Lipschitz regularity), there is a unique solution $(X,Y,Z)$ (see \cite{pard:rasc:14} for broad account on existence/uniqueness assumptions). Detailed hypotheses for the current study are exposed later.

Our aim in this article is to design a new numerical scheme for approximating the solution to the above BSDE. When $f$ is linear in $(Y,Z)$, explicit representations are available \cite[Theorem 1.1]{elka:peng:quen:97}, which can be easily turned into simple and efficient Monte-Carlo algorithms. Our focus is thus more on the case of non-linear driver yielding non-linear equations.

\paragraph{Feynman-Kac representations.} \red{Let us clearly show that FBSDEs are important tools in semi-linear PDEs and stochastic control theory.} Denote by  $\cal A$  the infinitesimal generator of $X$:
$$\cA =\sum_i b_i(t,x)\partial_{x_i}+\frac{1}{2 }\sum_{i,j} [\sigma \sigma^\top]_{i,j}(t,x)\partial^2_{x_i,x_j},$$
where $^\top$ denotes the transpose operator.
Consider the parabolic partial differential equation (PDE) of the form
\begin{equation}
\label{eq:pde}
\begin{cases}
\partial_{t}u(t,x)+{\cal A}u(t,x)+f(t,x,u(t,x),(\nabla_x u\sigma)(t,x))=0, \quad t<T,\\
u(T,.)=g(.).
\end{cases}
\end{equation}
Assuming that $u$ is smooth enough, the It\^o formula leads to 
$$u(t,X_t)=u(0,x)+\int_0^t (\partial_{t}u(s,X_s)+{\cal A}u(s,X_s))\ds+\int_0^t (\nabla_x u \sigma)(s,X_s) \dW_s.$$
Using the PDE \eqref{eq:pde} and noting $u(T,X_T)=g(X_T)$, we get
$$u(t,X_t)=g(X_T)+\int_t^T f(s,X_s,u(s,X_s), (\nabla_x u \sigma)(s,X_s) )\ds-\int_t^T (\nabla_x u \sigma)(s,X_s)  \dW_s,$$
therefore proving that the solution $(Y,Z)$ can be represented as
$$(Y_{t},Z_{t})=(u(t,X_t),(\nabla_{x} u\sigma) (t,X_{t})).$$
This is the well-known Feynman-Kac representation, making connection between semi-linear PDEs and BSDEs.  One may prefer one or the other representations depending on the application at hand, on the numerical scheme to use, and on the theoretical estimates available (of probabilistic or PDE nature). As a consequence,  solving numerically $(Y,Z)$ for any realization of $X$ or computing $(u,\nabla u)$ in the full space $\R^d$ gives, in both cases, essentially access to the same solution. The above reasoning holds for Cauchy boundary conditions and parabolic PDEs as presented above, however extensions in the directions of various boundary conditions (Dirichlet, Neumann, free-boundary) or stationary problems (elliptic PDEs) are also available, see \cite[Sections 3.8, 5.4, 5.6, 5.7 and 5.8]{pard:rasc:14} and references therein.

In view of \eqref{eq:pde}, the link with stochastic control appears  clearly, by analogy with the Hamilton-Jacobi-Bellman equation. Since the non-linearity in $f$ is related only to the first derivative of $u$ (the $Z$ component), the underlying control problem is associated to a control  in the drift only (not in the diffusion coefficient). See \cite{elka:peng:quen:97,elka:hama:mato:08} for some examples in finance.

\paragraph{Applications.} We now conclude the presentation of connection between BSDEs and PDEs by giving  a broader overview of applications where these semi-linear PDEs come into play. We follow the presentation of \cite[Section 7.1]{gobe:16}, some examples can be found in \cite[Chapter 2]{henr:81} and \cite[Chapter 14]{smol:94}.

\begin{description}
\item \emph{Ecology.} In a region of the plane ($d=2$), suppose the existence of  2 interacting species in the same environment and denote $u_k(t,x)$ ($k=1,2$) the population density of the individuals of each species at a point of the space $x$ and at a  time $t$. These population densities obey to the system
\begin{equation}
\label{eq:reac:diff:ecology}
\begin{cases}
\partial_t u_1(t,x) =\alpha_1 \Delta  u_1(t,x) +f_1(t,x,u_1,u_2),\\
\partial_t u_2(t,x) =\alpha_2 \Delta  u_2(t,x) +f_2(t,x,u_1,u_2), \quad t>0, x\in \R^2,\\
u_i(0,\cdot)\text{ {given}},
\end{cases}
\end{equation}
where the two Laplacian operators model the diffusive movement (as a Brownian motion) of each species. Note that the initial condition at $t=0$ can be turned into a terminal condition at $t=T$ as in our previous setting, this is just a simple 
time reversal  $t\leftrightarrow T-t$.

The  function $f=(f_1,f_2)$ plays the role of a growth rate of the population, describing the available local  resources and interactions between the species: the case $\partial_{u_2} f_1<0$ and $\partial_{u_1} f_2>0$ corresponds to the predator-prey model, where the growth rate of the species 1 (prey) decreases in the case of high density of the species 2 (predator) and conversely for the growth rate of predators; the case $\partial_{u_2} f_1>0$ and $\partial_{u_1} f_2>0$ models symbiosis, where each species benefits from the other;  $\partial_{u_2} f_1<0$ and $\partial_{u_1} f_2<0$ describes competition between species. This kind of model, introduced in the 30s by Fisher, Kolmogorov, Petrovsky and Piskunov, is discussed with extra references in \cite{shig:kawa:97}. 


\item \emph{Chemistry.} Suppose that a container contains $N$ chemical compounds taking part in $R$  independent reactions. Denote $c_i$ the concentration of the $i$-th {compound} and $\theta$ the temperature. Then their evolution  follows the $N+1$ equations (in $\R^+\times \R^3$)
\begin{equation}
\label{eq:reac:diff:chimie}
\begin{cases}
\varepsilon_p \partial_t c_i=D_i \Delta c_i+\sum_{j=1}^R \nu_{ij} g_j(c_1,\dots,c_N,\theta),\quad i=1,\dots,N,\\
\rho c_p \partial_t \theta = k \Delta \theta - \sum_{j=1}^R \sum_{i=1}^N\nu_{ij} H_i g_j(c_1,\dots,c_N,\theta),\\
c_i(0,\cdot)\text{ and }\theta(0,\cdot)\text{ {given}},
\end{cases}
\end{equation}
where $g_j$ is the speed of the $j$-th reaction and $H_i$ is the partial molar enthalpy of the $i$-th compound. For more details, see \cite{gava:68}. For reaction-diffusion equations, see \cite{smol:94}.

\item \emph{Neuroscience.} The famous model of Hodgkin and Huxley is a set of equations describing the psychological phenomenon of signal transmission in the axon (nerve fiber), showing the dependences between electrical excitability and various chemical ion concentrations. The PDE system is of  size $4$, the first unknown $u$ represents the electric potential and the three other unknowns $(v_1,v_2,v_3)$ are chemical concentrations: the system writes for $(t,x)\in \R^+\times \R $ (linear neuron)
\begin{equation}
\label{eq:reac:diff:neurosience}
\begin{cases}
c_0\partial_t u =\frac{ 1 }{R }  \partial^2_{xx }u +\kappa_1 v_1^3 v_2(c_1-u)+\kappa_2 v_3^4 (c_2-u)+\kappa_3 (c_3-u),\\
\partial_t v_1 =\varepsilon_1 \partial^2_{xx }  v_1 +g_1(u)(h_1(u)-v_1),\\
\partial_t v_2 =\varepsilon_2 \partial^2_{xx }  v_2 +g_2(u)(h_2(u)-v_2),\\
\partial_t v_3 =\varepsilon_3 \partial^2_{xx }  v_3 +g_3(u)(h_3(u)-v_3),\\
u(0,\cdot)\text{ and }v_i(0,\cdot)\text{ given},
\end{cases}
\end{equation}
for different positive constants $c_i, R, \kappa_i, \varepsilon_i$ and different functions $g_i,h_i$. There also exists a simplification of this model, known as the FitzHugh-Nagumo model. 

\item \emph{Materials physics.} The Allen-Cahn equation is a prototype model of  phase transition with a diffusive interface, used to model, for example, a solid/liquid phase transition \cite{visi:96}. The system is one-dimensional, and takes the form (in $\R^+\times \R^3$)
\begin{equation}
\label{eq:reac:diff:materiau}
\begin{cases}
\partial_t u =\varepsilon \Delta u + u(1-u^2),\\ 
u(0,\cdot) \text{ given.}
\end{cases}
\end{equation}
The solution $u$ thus represents an order parameter defining the arrangement of atoms in a crystal lattice.

\item \emph{Economy and finance.} There are numerous applications of BSDEs (and semi-linear PDEs) in finance, we refer the
reader to \cite{cvit:ma:96,elka:peng:quen:97,crep:13}. Let us mention:  valuation/hedging of contingent claim in complete markets; some market imperfections, such as higher interest rate for borrowing
\cite{berg:95}; incomplete markets \cite{pham:09} or super-replication \cite{elka:quen:95};  connections with recursive utilities in \cite{duff:epst:92}; non-linear pricing rule \cite{peng:03:a}; \red{second order BSDEs (2BSDEs) \cite{cheri:mete:touz:vict:2006,soner:touz:zhang:2011} which provide a stochastic representation for solutions of fully non-linear parabolic PDEs through a driver depending also on another process directly connected with the Hessian of the solution of the corresponding PDE; reflected BSDEs, where the solution $Y$ is constrained to stay above a given process called obstacle, were introduced by El Karoui et al in \cite{karoui:kapo:pard:peng:quen97}, and combined with jumps are able to connect with partial-integro differential equations \cite{barles:buck:pard:97,delong:13}}, etc. See \cite{elka:hama:mato:08,crep:13} for extra references of applications in finance.
\end{description}




\paragraph{Numerical approximations.} In the two past decades, there have been
several attempts to design efficient approximation schemes for BSDEs. \red{First, the four step algorithm was proposed by Ma, Proter and Yong \cite{ma:protter:yong:94} in 1994 to solve general FBSDEs. Their method is based on the finite difference approximation of the associated quasilinear parabolic PDE, and therefore becomes unaffordable in high dimension. In 1997, a discrete scheme based on the approximation of the Brownian motion by some discrete process was proposed by Chevance in \cite{chev:97}, while Bally considered a random time scheme in \cite{ball:97}, although this method requires the computation of conditional expectations to become a fully implementable solver. } At that time, only time-discretization issue was considered. Since then, optimal discretization strategies have been derived: see \cite{geis:geis:gobe:12} and references therein. \red{All probabilistic approaches proposed later roughly follow three steps: time discretization, dynamic programming principle and computation of conditional expectations. The problem of discretization and simulation of the forward component $X$ is well-understood, one could use standard Euler scheme or other choices like Milstein scheme, see \cite{kloeden:platen:92}. The difficulty  lies in the backward component $Y$, since a naive discretization of the backward SDE in $Y$ is not guaranteed to be adapted. In order to obtain a computationally viable  backward induction scheme one should take conditional expectations}. If the time grid is $\{t_0:=0,\dots,t_i,\dots,t_N=:T\}$, it leads to a nested expectation problem of the form  (also called Dynamic Programming Equation, or DPE for short)\red{
\begin{align}
\label{eq:ODP:intro:a}
Z_{\ti}&\approx\Esp{ Y_{t_{i+1}} \frac{(W_\tip-W_\ti)^\top}{ \tip-\ti}\mid \cF_{\ti}},\\
\label{eq:ODP:intro:b}
Y_{T} = g(X_T), \quad Y_{\ti}&\approx\Esp{ Y_{t_{i+1}} + f(t_i,X_{\ti},Y_{\tip},Z_\ti) (\tip-\ti)\mid \cF_{\ti}},
\end{align}
for $i=N-1,\ldots,0$.} We use the symbol $\approx$ to emphasize the heuristics, a rigorous justification can be done using the aforementioned references. 
\red{The scheme \eqref{eq:ODP:intro:a}-\eqref{eq:ODP:intro:b}, which is known as one-step forward dynamic programming scheme, could be updated taking into account a resimulation of the forward process till maturity, thus resulting in the so-called multi-step forward dynamic programming scheme, which is written as follows}
\begin{align}
\label{eq:MDP:intro:0a}
Z_{\ti}&\approx\Esp{ \bigg(g(X_T) +\sum_{j=i+1}^{N-1}f(t_j,X_{\tj},Y_{\tjp},Z_\tj) (\tjp-\tj)\bigg) \frac{(W_\tip-W_\ti)^\top}{ \tip-\ti}\mid \cF_{\ti}},\\
\label{eq:MDP:intro:0b}
Y_{\ti}&\approx\Esp{ g(X_T) +\sum_{j=i}^{N-1}f(t_j,X_{\tj},Y_{\tjp},Z_\tj) (\tjp-\tj)\mid \cF_{\ti}},
\end{align}
for $i=N-1,\ldots,0$. 
\red{\\Analytically, both schemes \eqref{eq:ODP:intro:a}-\eqref{eq:ODP:intro:b} and \eqref{eq:MDP:intro:0a}-\eqref{eq:MDP:intro:0b} are equivalent. However, differences arise when conditional expectations are numerically approximated. In fact, the multi-step scheme leads to better error estimates of the solutions computed by the developed algorithms, see \cite{gobe:turk:2016}.}
The above backward dynamic programming equations make clearly appear that at each of $N$ grid times, one has to compute a conditional expectation function, that is a function from $\R^d$ to $\R$, this is in a way equivalent to solving the PDE at each time point $t_i$. This is a difficult problem, with increasing difficulty as the dimension gets large and/or as the unknown function gets less smooth (\emph{curse of dimensionality}), like for finite differences schemes  for PDEs. Among the numerous approaches, let us mention 
the quantization method of Bally and Pag\`es \cite{ball:page:03}, which is an optimal space discretization of the
underlying dynamic programming equation, suitable to compute easily the conditional expectations on the space grid; in  \cite{bouc:touz:04} the authors compute the regression function with Malliavin calculus integration by parts combined with Monte Carlo simulations; the use of empirical regression methods and machine learning techniques is developed in \cite{gobe:lemo:wari:05,lemo:gobe:wari:06} (also called \emph{regression Monte-Carlo method}). Optimal convergence rates with regression methods are derived in \cite{gobe:turk:2016}.

\red{Recently, Henry-Labordere et al. \cite{henr:tan:touz:14} and Bouchard et al. \cite{bouc:tan:warin:zou:2017} proposed a branching method and a time step randomization applied to the Feynman-Kac representation of the PDE. Although branching techniques really overcome the curse of dimensionality, unfortunately they are only limited to small maturities, some small non-linearities and mainly to non-linearities that are polynomial in the solution and its gradient. Lately, in \cite{wei:jie:jentzen:2017} the authors propose a deep learning technique, referred as deep BSDE, to solve semi-linear PDEs or the corresponding BSDEs. They interpret the BSDE as a stochastic control problem with the gradient of the solution being the policy function, which is approximated or learned by a deep neural network, as has been done in deep reinforcement learning. More precisely, after discretizing the forward SDE in $X$ using Euler discretization, the algorithm reads the BSDE for $Y$ as a forward SDE, and the method tries to learn the value of $Y$ and $Z$ at each time step of the Euler scheme by minimizing a global loss function between the forward simulation of $Y$ until the maturity $T$ and the goal $g(X_T)$. In the recent work \cite{cwn:mik:warin:2019}, the authors give an improved version of the deep BSDE method, where a fixed point problem is solved using deep learning techniques. Machine learning techniques for high dimensional PDEs is nowadays a very active area of research \cite{hure:pham:achref:langrene:2018a,hure:pham:achref:langrene:2018b,hure:pham:warin:2019}. Numerical results show that these kind of algorithms are able to solve accurately problems in dimension $50$ and even above. However, these methods suffer so far from the lack of rigorous error estimates and the matter that convergence is not guaranteed. In fact, the approximation error goes to zero as long as the number of time steps and the number of neurons are increased, although only in the cases where the stochastic gradient descend method used to minimize the loss function is not trapped in a local minimum.}

\paragraph{Parallel computations.} Most of the above methods do not allow parallel computations because of the non-linearity of the equations. Recently in \cite{gltv}, the authors have proposed  a novel approach inspired from regression Monte-Carlo schemes suitable for massive parallelization, with excellent results on GPUs. It takes advantage of local approximations of the regression function in different strata of the state space $\R^d$ (partitioning estimates) and of a new stratified sampling scheme to guarantee that enough simulations are available in each stratum to compute accurately the regression functions. The parallelization step is made with respect to the strata. 


Our current work lies in this vein and is aimed at overcoming some drawbacks of the stratified regression scheme of \cite{gltv}. In the previous scheme, the solution $u$ to the PDE is represented as a piecewise polynomial function (like in a discontinuous Galerkin method \cite{dipi:ern:11}) and therefore, even if the exact solution is continuous, the approximation may be not, especially at the interface of the different strata. In the current work, we propose a different scheme, where the approximated solution is decomposed on basis functions that are smooth and that have natural orthonormal properties with respect to the sampling distribution, thus avoiding the possible discontinuity at the interfaces. Moreover, the sampling distribution is required to have some nice stability properties, useful for  the propagation of error in the DPE
%Dynamic Programming Equation
, see Theorem \ref{th:main}; we prove that the Student's t-distribution meets this requirement, see Theorem \ref{theo:uses}. One possible set of smooth and orthonormal functions is given by the trigonometric basis composed with a space transformation related to the Cumulative Distribution Function (CDF for short) of the Student's t-distribution. We call such a basis the \emph{Student-cosine basis}.
%
%
%\red{is decomposed on a trigonometric basis composed with a space transformation related to the Cumulative Distribution Function (CDF) of Student's t-distribution}% (the polynomial-based method is also known as spectral method)
%, thus avoiding the possible discontinuity at the interfaces. \red{We call such a basis the \emph{Student-cosine basis}. The Student distribution is used as a sampling distribution and this choice leads to nice stability properties for the propagation of error in the Dynamic Programming Equation (DPE), see Theorem \ref{th:main}.} 
Instead of a regression Monte Carlo scheme, we design a \emph{quasi-regression Monte-Carlo scheme}: we take advantage of the fact that  the basis functions enjoy orthonormal properties, in order to compute the basis coefficients as simple Monte-Carlo averages, instead of solutions of least-squares problems. On the one hand, it leads to a simplified and quicker procedure (because we avoid inverting linear systems). On the other hand, we obtain a globally smooth approximation which is mainly suitable for smooth solutions $u$ \cite{funaro,Canuto-Hussaini-Quarteroni-Zang}: this is a significant difference with partitioning estimates which can approximate well locally (ir-)regular functions. In this new scheme, the notion of strata is lost and the parallelization is now made with respect to the numerous required simulations and basis coefficients.
Moreover, we establish tight non-asymptotic error estimates (as a function of the size of the function basis and the number of Monte-Carlo simulations). 

In recent years, GPUs have become increasingly attractive for general purpose parallel computations. GPUs are not only impressive graphics tools but also highly parallel programmable processors that can deliver order-of-magnitude performance gains over optimized CPU applications. CPU hardware is designed to handle complex tasks, instead, GPUs only do one thing well, they handle millions of repetitive low level tasks. These high performance computing devices offer an arithmetic capability and a memory bandwidth that substantially outpace their CPU counterpart. In fact, a single NVIDIA Titan V GPU can sustain over 13.8 tera-floating-point operations per second (Tflops) and a memory bandwidth of 652.8 GB/s. In the last years GPUs have been heavily used in scientific computation in order to achieve dramatic runtime reductions over traditional CPU codes. Particularly successful applications of GPUs include Monte Carlo methods like the one we target in the present work. Indeed, Monte Carlo algorithms follow all design principles of GPU computing, they give rise to embarrassingly parallel not divergent codes that can exploit the GPU arithmetic intensity and its streaming memory bandwidth. In the last part of this article our goal is to offer an efficient implementation of the proposed algorithm taking advantage of several GPUs, which will allow us to address the solution of semi-linear PDEs in high dimensions.


\paragraph{Organization of the paper.} In Section \ref{section:Mathematical framework and basic properties}, we set the
framework of our study, define some notations used throughout the
paper and describe our algorithm based on the approximation of
conditional expectations by a projection on a finite orthonormal basis of
functions. Compared to the usual DPE %Dynamic Programming Equation (DPE for short) 
to solve \eqref{eq:MDP:intro}, we propose an equivalent modification that includes a weighted factor: this weight is related to the sampling distribution and its crucial purpose is to lead to higher order approximation of the unknown function under the condition it is smooth (see the Fourier-based analysis in Section \ref{sec:approError}). %Then, we analyze the approximation error due to the basis functions. 
Proofs of the propagation of error are postponed to Section \ref{section:error}. This new numerical scheme has been tested on GPU, which is exposed in Section \ref{section:GPU implementations}. Numerical results are collected in Section \ref{sec:numExperiments}.

\paragraph{Notations of the paper.} 
\begin{enumerate}[(i)]
 \item $\log(x)$ stands for the natural logarithm of $x\in \mathbb{R}_+$.
 \item $|\mb{x}|$ stands for the Euclidean norm of the vector $\mb{x}=(x_1,\dots, x_n)\in \R^n$.
 \item $\overline{\mb x}$ stands for the $l_1$-norm of the vector $\mb{x}=(x_1,\dots,x_n)\in\R^n$, i.e.\\$\overline{\mb x} = \norm{\mb{x}}_{1} = \sum_{i=1}^n |x_i|$. It will be mainly used when $x$ is a multi-index of integers used for differentiation.
 \item $(x)_+$ means the positive part of $x\in\R$ defined by $(x)_+ = \max(x,0)$.
 \item {$\Re{z}$ denotes the real part of the complex $z\in \mathbb{C}$; we set $\mb{i}:=\sqrt{-1}$.}
 \item For any finite $L>0$ and $\mb{x} = (x_1,\dots,x_n)\in \R^n$, define the soft truncation function
\begin{equation}
\nonumber%\label{eq:TL}
\cT_L(\mb{x}) := (-L\vee x_1 \wedge L, \dots, -L \vee x_n \wedge L).
\end{equation}
{Moreover, if $L:\R^n\to \R^+$ is a measurable function, then the above definition of $\cT_L$ is extended by replacing $L$ by $L(\mb{x})$:
\begin{equation}
\label{eq:TL:2}
\cT_L(\mb{x}) := (-L(\mb{x})\vee x_1 \wedge L(\mb{x}), \dots, -L(\mb{x}) \vee x_n \wedge L(\mb{x})).
\end{equation}}
{ \item Let $\mb{j}$, $\mb{k} \in \N^d$ be two multi-indices.  $\mb{j} \leq \mbk$ means that $j_l\leq k_l$ for all $l=1,\ldots,d$.
 \item  The finite multi-indices set $\Lambda\subset \N^d$ is downward closed if $$(\mbk\in\Lambda \mbox{ and } \mb{j} \leq \mbk) \Rightarrow \mb{j} \in\Lambda.$$
 \item Let ${\Lambda}\subset\N^d$ be an arbitrary downward closed multi-index set and $f:\R^d\rightarrow\R$. $f$ is ${\Lambda}$-smooth if ${\partial^{\mb{n}}_x} f$ exist and are continuous for all $\mb n\in {\Lambda}$.
 }
\end{enumerate}

